Leaky Buddies: Cross-Component Covert Channels on Integrated CPU-GPU Systems

Graphics Processing Units (GPUs) are a ubiquitous component across the range of today's computing platforms, from phones and tablets, through personal computers, to high-end server class platforms. With the increasing importance of graphics and video workloads, recent processors are shipped with GPU devices that are integrated on the same chip. Integrated GPUs share some resources with the CPU and as a result, there is a potential for microarchitectural attacks from the GPU to the CPU or vice versa. We believe this type of attack, crossing the component boundary (GPU to CPU or vice versa) is novel, introducing unique challenges, but also providing the attacker with new capabilities that must be considered when we design defenses against microarchitectrual attacks in these environments. Specifically, we consider the potential for covert channel attacks that arise either from shared microarchitectural components (such as caches) or through shared contention domains (e.g., shared buses). We illustrate these two types of channels by developing two reliable covert channel attacks. The first covert channel uses the shared LLC cache in Intel's integrated GPU architectures. The second is a contention based channel targeting the ring bus connecting the CPU and GPU to the LLC. Cross component channels introduce a number of new challenges that we had to overcome since they occur across heterogeneous components that use different computation models and are interconnected using asymmetric memory hierarchies. We also exploit GPU parallelism to increase the bandwidth of the communication, even without relying on a common clock. The LLC based channel achieves a bandwidth of 120 kbps with a low error rate of 2%, while the contention based channel delivers up to 400 kbps with a 0.8% error rate.

==> EXTRA/extra.tex <==
\subsection{Motivation for contention based channel}
%Intel name each of the components inside the SoC as the system agent. Each of the CPU code and the GPUs are named as system agent. 
The GPU and CPU share many hardware resources including ring based bi-directional interconnect and LLC. To study the effect of the memory request generated from GPU on CPU, we have performed an experiment. To carry out the experiment, two parallel threads are launched from the CPU using \textit{pthreads} and each one is pinned to separate physical cores to avoid any compute unit resource contention. One thread is responsible to do the memory load on the CPU side and another thread carry out the GPU kernel preparation and launch. On the GPU side, we have used 256 threads which is the maximum number of threads allowed in a single work group. On the CPU side, the memory is accessed using random pointer chasing mechanism. However, on the GPU side the data is accessed in a non-random fashion. In both CPU and GPU, the access has been done with an offset of a cacheline size of 64B. The data has been accessed only once from both the GPU and CPU to avoid the effect of the LLC cache and to take the effect of contention due the other resource sharing mainly due to ring interconnect. The data is averaged over 1000 number of execution to reduce the noise arising from system. Between two experiment reading, from the CPU side the data is cleared, using \textit{clflush} instruction.

Figure \ref{fig:cpu_laod_1} shows CPU memory access latency by varying the CPU buffer size for different GPU buffer size. In Figure~\ref{fig:cpu_laod_1}, the X axis is the data size of the CPU buffer and the Y-axis is the access latency of the buffer. Different colour lines in the graph indicates the CPU buffer access latency for over different GPU buffer size. 0 MB refers to the memory access latency by CPU without any GPU access. 
\begin{figure}[!htbp]
  \includegraphics[width=\linewidth]{IMAGES/CPU MEMORY LOAD GRAPH.jpg}
  \caption{CPU memory load characterization}
  \label{fig:cpu_laod_1}
\end{figure}
\FloatBarrier
It is observed from the graph, that the memory access latency of CPU is affected when GPU is accessing the memory at the same time. This is due to sharing of the data bus by simultaneous access from both CPU and GPU. Though the  data access delay is observable when the data size is small, both in CPU and GPU, the effect is not significant. But, if we compare the CPU buffer access latency (keeping the GPU buffer size 1 MB), we can observe as the CPU buffer size increases, access latency also increases over 50\% compared to no access from GPU. As the GPU memory request increases, the performance of the CPU memory access latency also decreases. Access time of 8 MB buffer is 3.537 ms when there is no interference from GPU. Now as the GPU memory access increases to 8 MB the access latency increases to 7.216 ms which is more the 2x slowdown. This study helps us in determining the fact that GPU memory access is affecting the CPU memory access latency due to the sharing of resources.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure \ref{fig:accessLatency} shows the access latency for the parameter configuration of \textit{CPU-1MB-GPU-2MB-WG-32}. The CPU RAM access latency for 1 MB data is measured as 5.21 microsecond. The LLC access time for 1 MB memory without the simultaneous GPU access is 4.72 microsecond. With the simultaneous GPU access the, average CPU LLC access latency is observed to 4.77 microsecond to 4.8 microsecond. There is an increase of 1\% - 8\% increase in the access latency due to simultaneous GPU access.


\hoda{If there is no clear justification for these plots in Figure~\ref{fig:busCov_2}, maybe it is better to report the highest BW and lowest error rate for this covert channel and save some space as well??}


\begin{figure}[htbp!]
  \includegraphics[width=\linewidth]{IMAGES/Bus_cov_access_time.jpg}
  \caption{CPU Access latency of 1 MB memory}
  \label{fig:accessLatency}
\end{figure}
\FloatBarrier
